Phase tracking based on GPGPU and applications in Planetary radio Science

This paper introduces a phase tracking method for planetary radio science research with computational algorithm implemented fo r NVIDIA GPUs. In contrast to the phase-locked loop (PPL) phase counting method used in traditional Doppler data processing, this method fits the tracking data signal into the shape expressed by the Taylor polynomial with optimal phase and amplitude coefficients. The Differential Evolution (DE) algorithm is employed for polynomial fitting. In order to cope with high computational intensity of the proposed phase tracking method, the graphics processing units (GPUs) are employed. As a result, the method estimates the instantaneous phase, frequency, derivative of frequency (line-of-sight acceleration) and the total count phase of different integration scales. This data can be further used in planetary radio science research to analyze the planetary occultation and gravitational fields. The method has been tested on MEX (Mars Express, ESA) and Chang'E 4 relay satellite (China) tracking data. In a real experiment with 400K data block size and $\sim$80,000 DE solver objective function evaluations we were able to acheive the target convergence threshold in 6.5 seconds and do real-time processing on NVIDIA GTX580 and 2$\times$ NVIDIA K80 GPUs, respectively. The precision of integral Doppler (60s) is 2 mrad/s and 4 mrad/s for MEX(3-way) and Chang'E 4 relay satellite(3-way) respectively.

==> images/mytest.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,704){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(946,1213){\makebox(0,0)[r]{\strut{}$0.02$}}%
      \csname LTb\endcsname%
      \put(946,1722){\makebox(0,0)[r]{\strut{}$0.04$}}%
      \csname LTb\endcsname%
      \put(946,2231){\makebox(0,0)[r]{\strut{}$0.06$}}%
      \csname LTb\endcsname%
      \put(946,2740){\makebox(0,0)[r]{\strut{}$0.08$}}%
      \csname LTb\endcsname%
      \put(946,3248){\makebox(0,0)[r]{\strut{}$0.1$}}%
      \csname LTb\endcsname%
      \put(946,3757){\makebox(0,0)[r]{\strut{}$0.12$}}%
      \csname LTb\endcsname%
      \put(946,4266){\makebox(0,0)[r]{\strut{}$0.14$}}%
      \csname LTb\endcsname%
      \put(946,4775){\makebox(0,0)[r]{\strut{}$0.16$}}%
      \csname LTb\endcsname%
      \put(1078,484){\makebox(0,0){\strut{}$0$}}%
      \csname LTb\endcsname%
      \put(2223,484){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%
      \put(3368,484){\makebox(0,0){\strut{}$4$}}%
      \csname LTb\endcsname%
      \put(4513,484){\makebox(0,0){\strut{}$6$}}%
      \csname LTb\endcsname%
      \put(5658,484){\makebox(0,0){\strut{}$8$}}%
      \csname LTb\endcsname%
      \put(6803,484){\makebox(0,0){\strut{}$10$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Phase uncertainty[rad]}}}%
      \put(3940,154){\makebox(0,0){\strut{}Integration time T(block length)[s] }}%
      \csname LTb\endcsname%
      \put(5816,4602){\makebox(0,0)[r]{\strut{} {\small $\sigma_{noise}{(T)} $}}}%
      \csname LTb\endcsname%
      \put(5816,4382){\makebox(0,0)[r]{\strut{} {\small $ R_3(T/2) $} }}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{mytest}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> images/plot_converg <==
#! /bin/bash
# $Id: timedat.dem,v 1.7 2003/10/28 05:35:54 sfeam Exp $
#
gnuplot << EOF
set terminal postscript eps color enhanced solid "Helvetica" 15 
set output "converg.eps"
#set terminal epslatex standalone lw 2 color 11
#set output "erf.tex"
#set title "Residual analysis"
#set style data fsteps
#set xlabel "Date and Time (UTC)"
#set label "Date and Time (UTC)" at screen 0.5,0.05 center front
#set timefmt "%d/%m/%y\t%H%M"
#set timefmt "%Y-%m-%dT%H:%M:%S"
#set yrange [ 0 : ]
#set xdata time
#set xrange [ "2015-07-15T12":"2015-07-15T20" ]
set y2label "Objective function value (correlation)"
set ylabel "Objective function value (Chi-square)"
set xlabel "Iterations"
set format y2 "%0.3e"
#set format x "%d/%m\n%H:%M"
set ytics nomirror
set y2tics
set grid
#set key left
set bmargin 5  #调整边框
plot '../data/converg1' using 2 with lp lw 2   axis x1y1 t 'Chi-square',\
    '../data/converg1' using (\$3-0.31830988618) with lp lw 2  axis x1y2 t 'correlation'

EOF


==> images/plot_rem_nos <==
#! /bin/bash
gnuplot << EOF
set terminal epslatex 
set output 'mytest.tex'
set grid 
set  xrange [ 0 : 10  ]
#set format y "%0.1e"
set xlabel 'Integration time T(block length)[s] '
set ylabel 'Phase uncertainty[rad]'
plot 0.05*sqrt(1/x) lw 3 t ' {\small $\sigma_{noise}{(T)} $}' , (1/(2**4*4!))*0.002*x**4 lw 3 t ' {\small $ R_3(T/2) $} '
#plot 1/x  lw 3 title '$\frac{1}{x}$'
EOF
rm gnulatex*
xelatex ~/document/latex/notouch/gnulatex
mv gnulatex.pdf rem_nos.pdf


==> images/plot_spectrum <==
#! /bin/bash
gnuplot << EOF
set terminal postscript eps color enhanced solid "Helvetica" 15 
set output "spectrum.eps"
set grid
#set format y "%0.1e"
set xlabel 'Freqency[rad/s] '
set ylabel 'Signal amplitude'
plot '../data/spectrum_line'  using 1:2   t 'signal without frequency change',\
     '../data/spectrum_mid'   using 1:2   t 'signal with slight frequency change',\
     '../data/spectrum_width' using 1:2   t 'signal with rapid frequency change'
EOF

